Flexible Keyword Spotting based on Homogeneous Audio-Text Embedding

Spotting user-defined/flexible keywords represented in text frequently uses an expensive text encoder for joint analysis with an audio encoder in an embedding space, which can suffer from heterogeneous modality representation (i.e., large mismatch) and increased complexity. In this work, we propose a novel architecture to efficiently detect arbitrary keywords based on an audio-compliant text encoder which inherently has homogeneous representation with audio embedding, and it is also much smaller than a compatible text encoder. Our text encoder converts the text to phonemes using a grapheme-to-phoneme (G2P) model, and then to an embedding using representative phoneme vectors, extracted from the paired audio encoder on rich speech datasets. We further augment our method with confusable keyword generation to develop an audio-text embedding verifier with strong discriminative power. Experimental results show that our scheme outperforms the state-of-the-art results on Libriphrase hard dataset, increasing Area Under the ROC Curve (AUC) metric from 84.21% to 92.7% and reducing Equal-Error-Rate (EER) metric from 23.36% to 14.4%.

==> sections/2_related_work.tex <==
\section{Related Work}
\label{sec:related_work}

With the recent advances in neural network technology, several approaches have been applied for keyword spotting task. \cite{Samragh2022ISW, Kundu2022HEiMDaLHE,Zhang2017HelloEK} have explored Convolutional Neural Network for fixed-keyword based KWS.
For user-defined KWS, one set of prior works \cite{flexible_kws2_asr_embedding, fixed_kws3_Triplet_Loss, Jung2022MetricLF} utilizes enrolled audio samples for user-defined keywords which is broadly refereed as query-by-example (QbyE) methods. \cite{dtw_embedding, dtw_embedding1} has used Dynamic time warping (DTW) \cite{dtw} sequence comparison approach to measure the similarity between the enrolled and the query audio. \cite{flexible_kws2_asr_embedding} has used an ASR model to obtain embeddings for enrolled and query audio and then used single aggregated embedding vector to make comparison which suffers from the loss of information due to dimensionality redcution.

Other set of works \cite{Shin2022LearningAA, nishu2023matching} for user-defined KWS includes approaches where keywords are enrolled in textual format. Our proposed method falls in this category. Our baseline \cite{Shin2022LearningAA} employs audio and text encoders to learn a pre-defined pattern which compromises the alignment flexibility hence producing sub-optimal results. Other baseline \cite{nishu2023matching} has tried using two independently trained audio and text encoders and then project both modalities in a common embedding space. For a small footprint model, this approach makes the learning from two different embedding spaces (audio and text respectively) to a common embedding space harder and hence the overall accuracy suffers. We have tackled this problem, by proposing a novel text encoder derived from the embedding learning space of audio encoder. 
